STORE: Self-Provisioning Storage-as-a-Service for Serverless Functions

Serverless computing provides on-demand elasticity, pay-per-use, and simplified deployment. However, serverless functions are typically stateless and depend on external storage services such as object stores or databases to exchange data or support stateful functions. Provisioning and configuring these storage systems still requires manual setup or declarative scripts, introducing complexity, slowing development, and increasing the risk of configuration errors. To address these challenges, in this paper, we introduce \textsc{STORE}, a self-provisioning storage architecture for serverless functions. STORE automatically selects the optimal storage backend and eliminates developer effort through zero-touch and zero-configuration provisioning, achieved by moving the self-provisioning logic to the platform level. Our evaluation results show that STORE reduces implementation effort by up to 84% compared to well-established Infrastructure-as-Code frameworks such as Terraform and Pulumi while maintaining low latency and linear scalability under realistic workloads, without introducing performance overhead.

==> backup/function_abstraction.tex <==
%%%%%%%%%%%%% ADD TABLE HERE %%%%%%%%%%%%%
\input{tables/data_model}
\subsection{STORE Abstraction Model}

The Storage Abstraction Model defines how STORE exposes a uniform interface to developers while hiding provider heterogeneity. It consists of four abstraction pillars: (i) a \emph{Function Code Abstraction} that exposes APIs to developers, requiring minimal interaction, (ii) \emph{Data Shape Abstraction} that map high-level structures to efficient provider operations, (iii) a \emph{Zero-Touch Configuration} contract that resolves connectivity and identity transparently, and (iv) \emph{Backwards Compatibility} through abstractions for existing libraries.

\paragraph{Function Code Abstraction}

STORE provides APIs, detailed in \cref{tab:functions}, that define a small set of operations across all storage shapes. 
These form a stable contract between functions and storage, allowing developers to write the same handler code (\cref{lst:store-example}) independently of the provider. At runtime, STORE resolves the provider and translates the operations into native calls, allowing developers to focus on function logic while the platform manages provisioning and configuration.



% Lets keep only what is related to STORE
\begin{listing}[t]
\centering
\begin{tcblisting}{
  listing engine=minted,
  minted language=kotlin,
  listing only,
  width=\linewidth,
  colframe=white,    
  colback=white,  
  left=-4pt,right=0pt,top=-5pt,bottom=-5pt,
  minted options={fontsize=\footnotesize,breaklines,breakanywhere},
  before=\relax,
  after=\relax,
}
lateinit var client: StoreClient

@DefaultSecurityLevel(SecurityLevel.WORKFLOW)
lateinit var map: StoreMap

fun handler(input: String): String {
    map.put("counter", (map.get<Long>("counter") ?: 0L) + 1)
    val response = client.store("testsimple", input.toByteArray())
    val retResponse = client.retrieve("testsimple")
    return retResponse.data.toString()
}
\end{tcblisting}
\caption{\textsc{STORE} Function Handler}
\label{lst:store-example}
\end{listing}


\paragraph{Data Shape Abstraction}

STORE defines data shapes such as \texttt{Blob}, \texttt{Row}, \texttt{Stream}, and \texttt{Map} that capture diverse storage semantics. 
Each shape is bound to a minimal set of verbs (e.g., \texttt{put}, \texttt{retrieve}, \texttt{store}), which are translated into provider-native operations by pluggable translators. This ensures portability across heterogeneous backends while minimizing serialization and translation overhead. 

\paragraph{Zero Touch Configuration}
STORE removes all manual configuration by injecting endpoints, workflow identifiers, and tokens at deployment time, and resolving them at runtime. 
STORE Client-SDK automatically discovers the active STORE-Service through environment variables and headers, enabling seamless storage access without developer setup. This contract ensures consistency across functions, workflows, and tenants.

\paragraph{Backwards Compatibility}
To support existing applications, STORE offers an Auto-Migration framework consisting of language-specific sidecar adapters that rebind existing client libraries (e.g., S3, MinIO, Cassandra) to the STORE API. These adapters preserve original method signatures but transparently redirect calls through STORE, allowing legacy code to benefit from dynamic selection and zero-touch provisioning without modification.


==> tables/data_model.tex <==

\begin{table*}[t]
\caption{Store APIs}
\label{tab:functions}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Function} & \textbf{Description} & \textbf{Location} \\ \midrule
\texttt{store(request): Response} & Client interface function that stores data, overloaded for file, table, and dynamic. & Interfaces  \\ 
\texttt{retrieve(request): Response} & Client interface function that retrieves data, overloaded for file, table, and dynamic. & Interfaces  \\ 
\texttt{put(key, value): dynamic} & Map interface function that stores data with serialization, permission-checks and concurrency-management. & Interfaces  \\ 
\texttt{get(key): dynamic} & Map interface function that retrieves data, with dynamic deserialization. & Interfaces  \\ 
\texttt{getIdentity(): List<Identity>} & Collects all identities that apply to an execution of a function. & Resolvers  \\ 
\texttt{getName(): String} & Resolves the current function name & Resolvers  \\ 
\texttt{getWorkflowName(): String?} & Resolves the current workflow name & Resolvers  \\ 
\texttt{locate(): String} & Resolves the responsible instance of the Service & Locators  \\ 
\bottomrule
\end{tabular}%
}
\end{table*}


